A Deep Learning Approach for Selective Relevance Feedback

Pseudo-relevance feedback (PRF) can enhance average retrieval effectiveness over a sufficiently large number of queries. However, PRF often introduces a drift into the original information need, thus hurting the retrieval effectiveness of several queries. While a selective application of PRF can potentially alleviate this issue, previous approaches have largely relied on unsupervised or feature-based learning to determine whether a query should be expanded. In contrast, we revisit the problem of selective PRF from a deep learning perspective, presenting a model that is entirely data-driven and trained in an end-to-end manner. The proposed model leverages a transformer-based bi-encoder architecture. Additionally, to further improve retrieval effectiveness with this selective PRF approach, we make use of the model's confidence estimates to combine the information from the original and expanded queries. In our experiments, we apply this selective feedback on a number of different combinations of ranking and feedback models, and show that our proposed approach consistently improves retrieval effectiveness for both sparse and dense ranking models, with the feedback models being either sparse, dense or generative.

==> figdefs/cnn.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\columnwidth]{figs/cnn.pdf}
\caption{
\small
A concrete realization of the encoding of the query-document pairs via the use of DRMM-based early interaction. Interaction vectors between each query term and a top-retrieved document are stacked to form a matrix. The corresponding matrices for each top-retrieved document are considered as separate channels of input data, which are passed through 2D convolutional filters.}
\label{fig:cnn}
\end{figure}

==> figdefs/overview.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figs/overview.png}
\caption{
\small
A schematic overview of the data-driven modeling of the decision function for selective relevance feedback.
}
\label{fig:overview}
\end{figure}

==> figdefs/vary_top_docs.tex <==
\begin{figure}[t]
\centering

\resizebox{0.9\columnwidth}{!}{
  \begin{tikzpicture}
      \begin{axis}[
        %   title={\large \textbf{(a)}},
          xlabel={\textbf{$k$}},
          ylabel={\textbf{MAP}},
          xmin=5, xmax=20,
          ymin=0.27, ymax=0.37,
          xtick={5,10,15,20},
          ytick={0.27,0.28,0.29,0.30,0.31,0.32,0.33,0.34,0.35,0.36,0.37},
          legend pos=north east,
          legend cell align={left},
          xmajorgrids=true,
          ymajorgrids=true,
          grid style=dashed,
      ]
      
      \addplot[
          line width=0.5mm,
          color=orange,
          mark=o,
          ]
          coordinates {(5,0.3017)(10,0.3049)(15,0.2956)(20,0.2911)};
    %   
      \addplot[
          line width=0.5mm,
          color=cyan,
          mark=o,
          ]
          coordinates {(5,0.2941)(10,0.3192)(15,0.3098)(20,0.2900)};
      %
      \addplot[
          line width=0.5mm,
          color=red,
          mark=o,
          ]
          coordinates {(5,0.3019)(10,0.3291)(15,0.3137)(20,0.2956)};
    %   
      \legend{\textbf{RLM}, \textbf{\darf-CNN-CC},\textbf{\darf-BERT-CC}}
      \end{axis}
  \end{tikzpicture}
% 
  \begin{tikzpicture}
      \begin{axis}[
        %   title={\textbf{(b)}},
          xlabel={\textbf{$k$}},
          ylabel={\textbf{MAP}},
          xmin=5, xmax=20,
          ymin=0.40, ymax=0.50,
          xtick={5,10,15,20},
          ytick={0.40,0.41,0.42,0.43,0.44,0.45,0.46,0.47,0.48,0.49,0.50},
          legend pos=north east,
          legend cell align={left},
          xmajorgrids=true,
          ymajorgrids=true,
          grid style=dashed,
      ]
       
       \addplot[
          line width=0.5mm,
          color=orange,
          mark=o,
          ]
          coordinates {(5,0.4302)(10,0.4321)(15,0.4319)(20,0.4267)};
        % 
      \addplot[
          line width=0.5mm,
          color=cyan,
          mark=o,
          ]
          coordinates
          {(5,0.4400)(10,0.4529)(15,0.4327)(20,0.4293)};
      %
      \addplot[
          line width=0.5mm,
          color=red,
          mark=o,
          ]
          coordinates {(5,0.4413)(10,0.4629)(15,0.4497)(20,0.4318)};
    %   
      \legend{\textbf{RLM},\textbf{\darf-CNN-CC},\textbf{\darf-BERT-CC}}
      \end{axis}
  \end{tikzpicture}
}

% \resizebox{0.5\columnwidth}{!}{
%   \begin{tikzpicture}
%       \begin{axis}[
%         %   title={\large \textbf{(a)}},
%           xlabel={\textbf{$k$}},
%           ylabel={\textbf{MAP}},
%           xmin=5, xmax=20,
%           ymin=0.19, ymax=0.27,
%           xtick={5,10,15,20},
%           ytick={0.19,0.20,0.21,0.22,0.23,0.24,0.25,0.26,0.27},
%           legend pos=north east,
%           xmajorgrids=true,
%           ymajorgrids=true,
%           grid style=dashed,
%       ]
       
%       \addplot[
%           line width=0.5mm,
%           color=cyan,
%           mark=o,
%           ]
%           coordinates {(5,0.2134)(10,0.2311)(15,0.2339)(20,0.2087)};
%       %
%       \addplot[
%           line width=0.5mm,
%           color=red,
%           mark=o,
%           ]
%           coordinates {(5,0.2302)(10,0.2310)(15,0.2415)(20,0.2131)};
%     %   
%       \legend{\textbf{\darf-CNN-CC},\textbf{\darf-BERT-CC}}
%       \end{axis}
%   \end{tikzpicture}
% }
\caption{
\small
Sensitivity of MAP on TREC-Robust (left) and TREC-DL (right) with respect to the number of top documents $k$ used for feedback. The number of feedback terms was tuned independently for each dataset, the optimal values being $30$ for TREC-Robust and $15$ for TREC-DL.
}
\label{fig:vary_k}
\end{figure}


==> tables/bm25_res.tex <==
% \begin{table*}[t]
% \centering
% \caption{
% % \small
% A comparison of the retrieval effectiveness between \darf~ and a set of unsupervised and supervised models. Note that the base retrieval models used here is a statistical model, BM25 and a neural re-ranker, MonoT5, respectively. We report MonoT5 results only on TREC-DL and \dev-small. The improvements of the best results obtained by \darf~(bold-faced) over others are statistically significant (p-value<$0.05$). Prediction accuracy is measured only for decision-based approaches; greyed out elsewhere.
% }
% \label{tab:bm25_res}

% \begin{adjustbox}{width=1\textwidth}
% \small
% \begin{tabular}{lll ccc|ccc|ccc}
% \toprule

% & &
% & \multicolumn{3}{c}{TREC-Robust} 
% & \multicolumn{3}{c}{TREC-DL}
% & \multicolumn{3}{c}{\dev} \\

% \cmidrule(r){4-6}
% \cmidrule(r){7-9}
% \cmidrule(r){10-12}

% Type & & Methods 
% & Accu & MAP & nDCG
% & Accu & MAP & nDCG
% & Accu & MAP & nDCG \\

% \midrule

% % \multirow{12}{*}{\begin{turn}{90}Baselines\end{turn}}
% \multirow{11}{*}{Baselines}
% & $a$ & RLM 
% & \nores & 0.2923 & 0.5783
% & \nores & 0.4321 & 0.6401
% & \nores & 0.2162 & 0.3542\\

% % & $b$ & \rrf
% % & \nores & 0.3008 & 0.5791
% % & \nores & 0.4337 & 0.6405
% % & \nores & 0.2187 & 0.3548 \\

% & $b$ & \rrf
% & \nores & 0.3106 & 0.5801
% & \nores & 0.4400 & 0.6417
% & \nores & 0.2243 & 0.3553 \\

% & $c$ & \nqc 
% & 0.7108 & 0.2906 & 0.5709
% & 0.7233 & 0.4283 & 0.6286
% & 0.7202 & 0.2076 & 0.3534 \\

% & $d$ & \wig 
% & 0.7211 & 0.2912 & 0.5715
% & 0.7159 & 0.4204 & 0.6259
% & 0.7156 & 0.2004 & 0.3469 \\

% & $e$ & \clarity 
% & 0.6974 & 0.2803 & 0.5622
% & 0.6722 & 0.4059 & 0.6044
% & 0.6841 & 0.1934 & 0.3352 \\

% & $f$ & \unqc 
% & 0.7414 & 0.2984 & 0.5786
% & 0.7277 & 0.4287 & 0.6300
% & 0.7280 & 0.2092 & 0.3540 \\

% & $g$ & \uwig 
% & 0.7451 & 0.3002 & 0.5795
% & 0.7204 & 0.4215 & 0.6261
% & 0.7200 & 0.2017 & 0.3483 \\

% & $h$ & \uclarity 
% & 0.7152 & 0.2843 & 0.5657
% & 0.6858 & 0.4068 & 0.6071
% & 0.6874 & 0.1956 & 0.3361 \\

% & $i$ & \idf 
% & 0.7361 & 0.2965 & 0.5781
% & 0.7584 & 0.4338 & 0.6411
% & 0.7469 & 0.2149 & 0.3538 \\

% & $j$ & \mcf
% & 0.7526 & 0.3018 & 0.5800
% & 0.7611 & 0.4392 & 0.6417
% & 0.7623 & 0.2216 & 0.3547 \\

% & $k$ & \afr 
% & 0.7902 & 0.3114 & 0.5813
% & 0.7835 & 0.4423 & 0.6421
% & 0.7701 & 0.2301 & 0.3573 \\

% \midrule

% % \multirow{4}{*}{\begin{turn}{90}Ours\end{turn}}
% \multirow{4}{*}{Ours}
% & $l$ & \darf(CNN$_{point}$) 
% & 0.7311 & 0.2931 & 0.5772
% & 0.7200 & 0.4272 & 0.6253
% & 0.7632 & 0.2244 & 0.3549 \\

% & $m$ & \darf(CNN$_{pair}$)
% & 0.7962 & 0.3192 & 0.5859
% & 0.7891 & 0.4529 & 0.6456
% & 0.7824 & 0.2339 & 0.3621 \\

% & $n$ & \darf(BERT$_{point}$)
% & 0.7823 & 0.3167 & 0.5842
% & 0.7867 & 0.4433 & 0.6432
% & 0.7749 & 0.2312 & 0.3586 \\

% & $o$ & \darf(BERT$_{pair}$)
% & \textbf{0.8149} & \textbf{0.3291} & \textbf{0.5900}
% & \textbf{0.8081} & \textbf{0.4629} & \textbf{0.6494}
% & \textbf{0.8006} & \textbf{0.2415} & \textbf{0.3690}\\

% \midrule

% & & ORACLE
% & & 0.3329 & 0.5935
% & & 0.4656 & 0.6521
% & & 0.2467 & 0.3719 \\

% \bottomrule
                       
% \end{tabular}
% \end{adjustbox}
% \end{table*}

==> tables/msmarco.tex <==
\begin{table*}[t]
\centering
\caption{
\small
% \inote{rewrite} A comparison of the retrieval effectiveness for \darf~and a set of unsupervised and supervised baselines. We report results for both a statistical model, BM25, and a neural re-ranker, MonoT5. Note that a MonoT5 re-ranked list is used only for TREC-DL and \dev. The improvements in the results obtained by \darf~(bold-faced) over the others are statistically significant (paired t-test with $p$<$0.05$). Prediction accuracy is reported only for decision-based approaches.
% \inote{statistical significance}
\sd{Effective performance of our proposed method, \darf, on the \dev~dataset.}
}
\label{tab:msmarco}

\begin{adjustbox}{width=1\textwidth}
\small
\begin{tabular}{@{}l@{~~}lcccc|cccc|cccc@{}}

\toprule

& 
& \multicolumn{4}{c}{BM25 top-1000}
& \multicolumn{4}{c}{MonoT5 re-ranked}
& \multicolumn{4}{c}{ColBERT-PRF re-ranked} \\

\cmidrule(r){3-6}
\cmidrule(r){7-10}
\cmidrule(r){11-14}

Type & Methods 
& Accuracy & MAP & nDCG@10 & RR@10
& Accuracy & MAP & nDCG@10 & RR@10
& Accuracy & MAP & nDCG@10 & RR@10 \\

\midrule

\multirow{6}{*}{\begin{turn}{90}Baselines\end{turn}}
& No-feedback
& N/A & 0.1924 & 0.2296 & 0.1835
& N/A & 0.3800 & 0.4387 & 0.3761
& N/A & 0.3138 & 0.3887 & 0.3983\\

& PRF 
& N/A & 0.2148 & 0.2474 & 0.1842
& N/A & 0.3901 & 0.4429 & 0.3769
& N/A & 0.3219 & 0.3911 & 0.4120 \\

& \rrf
& N/A & 0.2243 & 0.2481 & 0.1843
& N/A & 0.3938 & 0.4438 & 0.3775
& N/A & 0.3222 & 0.3917 & 0.4126 \\

& \qppbert
& 0.7701 & 0.2287 & 0.2492 & 0.1846
& 0.7682 & 0.3981 & 0.4457 & 0.3785
& \underline{0.7944} & \underline{0.3304} & \underline{0.4011} & \underline{0.4162} \\

& \mcf
& 0.7623 & 0.2216 & 0.2431 & 0.1830
& 0.7758 & 0.3847 & 0.4391 & 0.3765
& 0.7482 & 0.3197 & 0.3824 & 0.4033 \\

& \afr 
& \underline{0.7756} & \underline{0.2297} & \underline{0.2496} & \underline{0.1848}
& \underline{0.7803} & \underline{0.4003} & \underline{0.4473} & \underline{0.3800}
& 0.7829 & 0.3267 & 0.3966 & 0.4138 \\

\midrule

\multirow{8}{*}{\begin{turn}{90}Ours\end{turn}}

& \darfcnn-point
& \\

& \darfcnn
& \multirow{3}{*}{0.7824} & 0.2300 & 0.2496 & 0.1842
& \multirow{3}{*}{0.7900} & 0.4020 & 0.4485 & 0.3821
& \multirow{3}{*}{0.7972} & 0.3315 & 0.4026 & 0.4170 \\

& \darfcnn-\rrf
& & 0.2339 & 0.2508 & 0.1850
& & 0.4082 & 0.4511 & 0.3852
& & 0.3352 & 0.4073 & 0.4177 \\

& \darfcnn-CC
& & 0.2412 & 0.2538 & 0.1862
& & 0.4101 & 0.4519 & 0.3873
& & 0.3361 & 0.4081 & 0.4200 \\

\cmidrule(r){2-2}

& \darfbert

& \multirow{3}{*}{\textbf{0.8006}$^*$} & 0.2437 & 0.2582 & 0.1886
& \multirow{3}{*}{\textbf{0.8014}$^*$} & 0.4186 & 0.4544 & 0.3901
& \multirow{3}{*}{\textbf{0.8081}$^*$} & 0.3330 & 0.4054 & 0.4181 \\

& \darfbert-\rrf
& & 0.2462 & 0.2591 & 0.1891
& & 0.4225 & 0.4558 & 0.3935
& & 0.3401 & 0.4071 & 0.4203 \\

& \darfbert-CC
& & \textbf{0.2526}$^*$ & \textbf{0.2619}$^*$ & \textbf{0.1915}$^*$
& & \textbf{0.4307}$^*$ & \textbf{0.4586}$^*$ & \textbf{0.3951}$^*$
& & \textbf{0.3427}$^*$ & \textbf{0.4077}$^*$ & \textbf{0.4236}$^*$ \\

\midrule

& Oracle
& \cellcolor{ashgrey}1.0000 & \cellcolor{ashgrey}0.2567 & \cellcolor{ashgrey}0.2680 & \cellcolor{ashgrey}0.1942
& \cellcolor{ashgrey}1.0000 & \cellcolor{ashgrey}0.4394 & \cellcolor{ashgrey}0.4621 & \cellcolor{ashgrey}0.3989
& \cellcolor{ashgrey}1.0000 & \cellcolor{ashgrey}0.3500 & \cellcolor{ashgrey}0.4108 & \cellcolor{ashgrey}0.4261 \\

\bottomrule
                       
\end{tabular}
\end{adjustbox}
\end{table*}

==> tables/res_tab_merge.tex <==
\begin{table*}[!ht]
\caption{
\small
caption
\label{tab:dl_and_dev}
}
\begin{subtable}[t]{0.8\linewidth}
\centering
\begin{adjustbox}{width=\textwidth}
\input{tables/trecdl.tex}
\end{adjustbox}
\caption{\small TREC-DL
\label{stab:tab_dl}
}
\end{subtable}%
\quad
\begin{subtable}[t]{0.8\linewidth}
\centering
\begin{adjustbox}{width=\textwidth}
\input{tables/msmarco.tex}
\end{adjustbox}
\caption{\small msmarco-dev
\label{stab:tab_dev}
}
\end{subtable}

\end{table*}

==> tables/robust.tex <==
\begin{table}[t]
\centering
\caption{
\small
%\sd{
Comparisons between the retrieval effectiveness for \darf~and a set of unsupervised and supervised baselines on the TREC-Robust dataset. BM25 is used as the initial retrieval model, and the PRF method employed is RLM. The improvements in the results obtained by \darf~(bold-faced) over the best performing baseline \afr~(underlined) are statistically significant (paired $t$-test with $p$<$0.05$ ). Results that are significantly improved over the baseline are marked with a ($*$) and we follow this convention for Table \ref{tab:trecdl} as well. Note that prediction accuracy is reported only for decision-based approaches in all the result tables (Table \ref{tab:robust} and \ref{tab:trecdl}); its value being `N/A' elsewhere.}
%}
\label{tab:robust}

\begin{adjustbox}{width=0.8\columnwidth}
\small
\begin{tabular}{@{}llcccc@{}}

\toprule

& 
& \multicolumn{4}{c}{BM25 top-1000} \\

\cmidrule(r){3-6}

Type & Methods 
& Accuracy & MAP & P@20 & nDCG@20 \\

\midrule

\multirow{6}{*}{\begin{turn}{30}Baselines\end{turn}}
& No PRF
& N/A & 0.2581 & 0.3673 & 0.4267 \\

& PRF 
& N/A & 0.3049 & 0.3968 & 0.4495 \\

& \rrf
& N/A & 0.3106 & 0.4011 & 0.4489 \\

% & \idf 
% & 0.7361 & 0.2965 & 0.0000 & 0.4411 \\

% & \unqc 
% & 0.7414 & 0.2984 & 0.0000 & 0.4532 \\

& \qppbert
& 0.7902 & 0.3189 & 0.4127 & 0.4580 \\

& \mcf
& 0.7526 & 0.3018 & 0.3960 & 0.4498 \\

& \afr 
& \underline{0.7935} & \underline{0.3218} & \underline{0.4134} & \underline{0.4586} \\

\midrule

\multirow{3}{*}{\begin{turn}{30}Ours\end{turn}}

%& \darfcnn-NoQE 
%& 0.7697 & 0.3062 & 0.3973 & 0.4498\\

% & \darfcnn
% & \multirow{3}{*}{0.7972} & 0.3203 & 0.4190 & 0.4677 \\

% & \darfcnn-\rrf
% & & 0.3227 & 0.4211 & 0.4680 \\

% & \darfcnn-CC
% & & 0.3292 & 0.4257 & 0.4681 \\

% \cmidrule(r){2-2}

%& \darfbert-NoQE 
%& 0.7714 & 0.3071 & 0.3944 & 0.4509\\

& \darfbert
& \multirow{3}{*}{\textbf{0.8149}$^*$} & 0.3273 & 0.4220 & 0.4673 \\

& \darfbert-\rrf
& & 0.3311 & 0.4234 & 0.4691 \\

& \darfbert-CC
& & \textbf{0.3391}$^*$ & \textbf{0.4281}$^*$ & \textbf{0.4719}$^*$ \\

\midrule

\multirow{3}{*}{\begin{turn}{30}Ablation\end{turn}}
% & \darfcnn-CC-NoQE 
% & 0.7697 & 0.3062 & 0.3973 & 0.4498\\
& \darfbert-CC-NoQE 
& 0.7714 & 0.3071 & 0.3944 & 0.4509 \\
\multicolumn{6}{c}{}\\

\midrule

& Oracle
& \cellcolor{ashgrey}1.0000 & \cellcolor{ashgrey}0.3429 & \cellcolor{ashgrey}0.4313 & \cellcolor{ashgrey}0.4749
\\

\bottomrule
                       
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/t5_res.tex <==
% \begin{table*}[t]
% \centering
% \caption{
% % \small
% Comparisons of the retrieval effectiveness between \darf~ and other baselines (similar to Table \ref{tab:bm25_res}), the difference being that the experiments are conducted on a neural model, specifically MonoT5, generated ranked list of documents. Best results are bold-faced and statistically significant (p-value<$0.05$) when compared to other models (row $i-xiv$)
% }
% \label{tab:t5_res}

% \begin{adjustbox}{width=0.7\textwidth}
% \small
% \begin{tabular}{lll ccc|ccc}
% \toprule

% & &
% & \multicolumn{3}{c}{TREC-DL}
% & \multicolumn{3}{c}{\dev} \\

% \cmidrule(r){4-6}
% \cmidrule(r){7-9}

% Type & & Methods 
% & Accu & MAP & ndcg
% & Accu & MAP & ndcg \\

% \midrule

% % \multirow{12}{*}{\begin{turn}{90}Baselines\end{turn}}
% \multirow{11}{*}{Baselines}
% & $i$ & RLM 
% & \nores & 0.5165 & 0.7091
% & \nores & 0.3901 & 0.4964 \\

% & $ii$ & \rrf
% & \nores & 0.5192 & 0.7095
% & \nores & 0.3938 & 0.4972 \\

% & $iii$ & \nqc 
% & 0.7364 & 0.4911 & 0.6838
% & 0.7412 & 0.3800 & 0.4813 \\

% & $iv$ & \wig 
% & 0.7111 & 0.4637 & 0.6513
% & 0.7236 & 0.3604 & 0.4582 \\

% & $v$ & \clarity 
% & 0.6913 & 0.4579 & 0.6404
% & 0.7041 & 0.3500 & 0.4492 \\

% & $vi$ & \unqc 
% & 0.7400 & 0.4918 & 0.6840
% & 0.7552 & 0.3810 & 0.4819 \\

% & $vii$ & \uwig 
% & 0.7189 & 0.4641 & 0.6534
% & 0.7164 & 0.3611 & 0.4625 \\

% & $viii$ & \uclarity 
% & 0.7034 & 0.4600 & 0.6410
% & 0.7060 & 0.3506 & 0.4500 \\

% & $ix$ & \idf 
% & 0.7432 & 0.4952 & 0.6861
% & 0.7639 & 0.3841 & 0.4839 \\

% & $x$ & \mcf
% & 0.7789 & 0.5171 & 0.7062
% & 0.7758 & 0.3847 & 0.4878 \\

% & $xi$ & \afr 
% & 0.7963 & 0.5200 & 0.7104
% & 0.7803 & 0.3883 & 0.4916 \\

% \midrule

% % \multirow{4}{*}{\begin{turn}{90}Ours\end{turn}}
% \multirow{4}{*}{Ours}
% & $xii$ & \darf(CNN$_{point}$) 
% & 0.7703 & 0.5100 & 0.7006
% & 0.7621 & 0.3822 & 0.4912 \\

% & $xiii$ & \darf(CNN$_{pair}$)
% & 0.8009 & 0.5217 & 0.7121
% & 0.7900 & 0.3927 & 0.4986 \\

% & $xiv$ & \darf(BERT$_{point}$)
% & 0.7910 & 0.5176 & 0.7100
% & 0.7881 & 0.3914 & 0.4923 \\

% & $xv$ & \darf(BERT$_{pair}$)
% & \textbf{0.8152} & \textbf{0.5249} & \textbf{0.7161}
% & \textbf{0.8014} & \textbf{0.4007} & \textbf{0.5022} \\

% \midrule

% & & ORACLE
% & & 0.5276 & 0.7200
% & & 0.4054 & 0.5091 \\

% \bottomrule
                       
% \end{tabular}
% \end{adjustbox}
% \end{table*}

==> tables/time.tex <==
\begin{table}[t]
\centering
\caption{
\small
Comparison of performance of two data-driven approaches (CNN and BERT both with `CC' and `NoQE') in terms of total training and per query inference times taken for $3$ datasets (similar to all our PRF experiments, the number of top-documents used for PRF is set to $10$). The training time reported is for 1 epoch and the batch size is set to $5$ in all cases. 
}
\label{tab:time}

\begin{adjustbox}{width=0.92\columnwidth}
% \small
\begin{tabular}{@{}ll ccccc@{}}
\toprule

\multirow{2}{*}{Dataset}
& \multirow{2}{*}{Methods}
& \multirow{2}{*}{\#Topics}
& \multicolumn{2}{c}{Training (min.)}
& \multicolumn{2}{c}{Inference (sec.)} \\

\cmidrule{4-5}
\cmidrule{6-7}

& & 
& CC & NoQE
& CC & NoQE \\

\midrule

\multirow{2}{*}{TREC-Robust}
& \darf-CNN
& \multirow{2}{*}{249}
& 1.07 & 1.03 & 0.32 & 0.27 \\

& \darf-BERT &
& 3.58 & 3.35 & 1.07 & 1.01 \\

\cmidrule{2-7}

\multirow{2}{*}{TREC-DL}
& \darf-CNN
& \multirow{2}{*}{97}
& 0.42 & 0.39 & 0.33 & 0.31 \\

& \darf-BERT &
& 1.43 & 1.38 & 1.02 & 1.00 \\

\cmidrule{2-7}

\multirow{2}{*}{Dev-small}
& \darf-CNN
& \multirow{2}{*}{6980}
& 211 & 207 & 0.32 & 0.30 \\

& \darf-BERT &
& 713 & 702 & 1.06 & 1.02 \\

\bottomrule
                       
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/trecdl.tex <==
\begin{table*}[t]
\centering
\caption{
\small
% Similar to Table \ref{tab:robust} the retrieval effectiveness of \darf~is shown on TREC-DL dataset. We report results for both a statistical model, BM25, and a neural re-ranker, MonoT5. Note that MonoT5 re-ranked list is used only for TREC-DL and \dev. The improvements for the best results obtained by \darf~(bold-faced) over the others are statistically significant (paired t-test with $p$<$0.05$). Prediction accuracy is reported only for decision-based approaches.
%\sd{
A comparative evaluation of different SRF approaches on the TREC DL (2019 and 2020) and MS MARCO Dev-small topic sets.
%Similar to Table \ref{tab:robust}, the retrieval effectiveness of the proposed \darf~approaches are compared with the baselines.
%These results evaluated on TREC-DL dataset here.
In addition to BM25, we report results with dense neural IR models, MonoT5 and ColBERT.
The PRF method used for improving the ColBERT results is ColBERT-PRF, whereas for BM25 and MonoT5 results are reported with RLM as the PRF method.
%Note that MonoT5 and ColBERT re-ranked list is used only for TREC-DL and \dev~(see Table \ref{tab:msmarco}).
Paired $t$-test ($p$<$0.05$) shows a significant improvement of \darf~over the best performing baselines (comparing bold-faced results with the underlined ones).
%}
% \inote{statistical significance}
}
\label{tab:trecdl}

\begin{adjustbox}{width=0.95\textwidth}
\small
\begin{tabular}{@{}llcccc|cccc|cccc@{}}

\toprule
\multicolumn{13}{c}{\textbf{Topic Set: TREC DL 19 and 20}} \\
\midrule
& 
& \multicolumn{4}{c}{BM25 ($\phi$: RLM)}
& \multicolumn{4}{c}{MonoT5 ($\phi$: RLM)}
& \multicolumn{4}{c}{ColBERT ($\phi$: ColBERT-PRF)} \\

\cmidrule(r){3-6}
\cmidrule(r){7-10}
\cmidrule(r){11-14}

& Methods 
& Accuracy & MAP & nDCG@10 & RR@10
& Accuracy & MAP & nDCG@10 & RR@10
& Accuracy & MAP & nDCG@10 & RR@10\\

\midrule

\multirow{6}{*}{\begin{turn}{30}Baselines\end{turn}}
& No PRF 
& N/A & 0.3766 & 0.5022 & 0.7791
& N/A & 0.5062 & 0.6451 & 0.8847
& N/A & 0.4770 & 0.7125 & 0.8723 \\


& PRF 
& N/A & 0.4321 & 0.5134 & 0.7720
& N/A & 0.5081 & 0.6463 & 0.8826
% & N/A & 0.5072 & 0.7172 & 
& N/A & 0.5014 & 0.7167 & 0.8729 \\

& \rrf
& N/A & 0.4381 & 0.5140 & 0.7789
& N/A & 0.5112 & 0.6484 & 0.8827
& N/A & 0.5168 & 0.7184 & 0.8735\\

% & \idf 
% & 0.7584 & 0.4338 & 0.5136
% & 0.7432 & 0.4952 & 0.6449
% & 0.7309 & 0.5063 & 0.6784 \\

% & \unqc 
% & 0.7277 & 0.4287 & 0.4891
% & 0.7400 & 0.4918 & 0.6322
% & 0.7277 & 0.5018 & 0.6604 \\

& \qppbert
& 0.7835 & 0.4400 & 0.5152 & 0.7800
& \underline{0.7963} & \underline{0.5189} & \underline{0.6559} & \underline{0.8854}
& 0.7742 & 0.5238 & 0.7200 & 0.8742 \\

& \mcf
& 0.7611 & 0.4392 & 0.5135 & 0.7703
& 0.7789 & 0.5071 & 0.6453 & 0.8812
& 0.7642 & 0.5210 & 0.7138 & 0.8733\\

& \afr 
& \underline{0.7842} & \underline{0.4411} & \underline{0.5154} & \underline{0.7800}
& 0.7958 & 0.5180 & 0.6543 & 0.8847
& \underline{0.7854} & \underline{0.5254} & \underline{0.7214} & \underline{0.8748}\\

\midrule

\multirow{3}{*}{\begin{turn}{30}Ours\end{turn}}

% & \darfcnn
% & \multirow{3}{*}{0.7891} & 0.4448 & 0.5196 & 0.7821
% & \multirow{3}{*}{0.8009} & 0.5204 & 0.6583 & 0.8871
% & \multirow{3}{*}{0.8044} & 0.5309 & 0.7222 & 0.8756 \\

% & \darfcnn-\rrf
% & & 0.4512 & 0.5201 & 0.7828
% & & 0.5217 & 0.6597 & 0.8878
% & & 0.5381 & 0.7230 & 0.8760\\

% & \darfcnn-CC
% & & 0.4571 & 0.5243 & 0.7831
% & & 0.5253 & 0.6608 & 0.8885
% & & 0.5402 & 0.7253 & 0.8779 \\

% \cmidrule(r){2-2}

& \darfbert
& \multirow{3}{*}{\textbf{0.8081}$^*$} & 0.4605 & 0.5274 & 0.7858
& \multirow{3}{*}{\textbf{0.8152}$^*$} & 0.5306 & 0.6640 & 0.8903
& \multirow{3}{*}{\textbf{0.8165}$^*$} & 0.5431 & 0.7265 & 0.8784 \\

& \darfbert-\rrf
& & 0.4661 & 0.5286 & 0.7873
& & 0.5317 & 0.6659 & 0.8910
& & 0.5485 & 0.7273 & 0.8791 \\

% & \darfbert-CC
% & & \textbf{0.4692}$^*$ & \textbf{0.5303}$^*$ & \textbf{0.7896}$^*$
% & & \textbf{0.5383}$^*$ & \textbf{0.6671}$^*$ & \textbf{0.8922}$^*$
% & & \textbf{0.5511}$^*$ & \textbf{0.7292}$^*$ & \textbf{0.8801}$^*$\\

\midrule

\multirow{2}{*}{\begin{turn}{30}Ablations\end{turn}}
& \darfbert-CC-NoQE
& 0.7694 & 0.4418 & 0.5126 & 0.7750
& 0.7820 & 0.5200 & 0.6511 & 0.8847
& 0.7769 & 0.5248 & 0.7190 & 0.8738\\

& \darfcnn-CC-NoQE
& 0.7600 & 0.4363 & 0.5137 & 0.7746
& 0.7793 & 0.5118 & 0.6493 & 0.8831
& 0.7692 & 0.5216 & 0.7191 & 0.8735 \\

\midrule

& Oracle
& \cellcolor{ashgrey}1.0000 
& \cellcolor{ashgrey}0.4738 
& \cellcolor{ashgrey}0.5328 
& \cellcolor{ashgrey}0.7903
& \cellcolor{ashgrey}1.0000 
& \cellcolor{ashgrey}0.5416 
& \cellcolor{ashgrey}0.6686
& \cellcolor{ashgrey}0.8937
& \cellcolor{ashgrey}1.0000 
& \cellcolor{ashgrey}0.5542 
& \cellcolor{ashgrey}0.7336
& \cellcolor{ashgrey}0.8811\\

\bottomrule
                       
\end{tabular}
\end{adjustbox}



% Dev
% \begin{adjustbox}{width=0.95\textwidth}
% \small
% \begin{tabular}{@{}llcccc|cccc|cccc@{}}

% \toprule

% \multicolumn{13}{c}{\textbf{Topic Set: MS MARCO Dev-small}} \\
% \midrule

% & 
% & \multicolumn{4}{c}{BM25 ($\phi$: RLM)}
% & \multicolumn{4}{c}{MonoT5 ($\phi$: RLM)}
% & \multicolumn{4}{c}{ColBERT ($\phi$: ColBERT-PRF)} \\

% \cmidrule(r){3-6}
% \cmidrule(r){7-10}
% \cmidrule(r){11-14}

%  & Methods 
% & Accuracy & MAP & nDCG@10 & RR@10
% & Accuracy & MAP & nDCG@10 & RR@10
% & Accuracy & MAP & nDCG@10 & RR@10 \\

% \midrule

% \multirow{6}{*}{\begin{turn}{30}Baselines\end{turn}}
% & No PRF
% & N/A & 0.1924 & 0.2296 & 0.1835
% & N/A & 0.3800 & 0.4387 & 0.3761
% & N/A & 0.3138 & 0.3887 & 0.3983\\

% & PRF 
% & N/A & 0.2148 & 0.2474 & 0.1842
% & N/A & 0.3901 & 0.4429 & 0.3769
% & N/A & 0.3219 & 0.3911 & 0.4120 \\

% & \rrf
% & N/A & 0.2243 & 0.2481 & 0.1843
% & N/A & 0.3938 & 0.4438 & 0.3775
% & N/A & 0.3222 & 0.3917 & 0.4126 \\

% & \qppbert
% & 0.7701 & 0.2287 & 0.2492 & 0.1846
% & 0.7682 & 0.3981 & 0.4457 & 0.3785
% & \underline{0.7944} & \underline{0.3304} & \underline{0.4011} & \underline{0.4162} \\

% & \mcf
% & 0.7623 & 0.2216 & 0.2431 & 0.1830
% & 0.7758 & 0.3847 & 0.4391 & 0.3765
% & 0.7482 & 0.3197 & 0.3824 & 0.4033 \\

% & \afr 
% & \underline{0.7756} & \underline{0.2297} & \underline{0.2496} & \underline{0.1848}
% & \underline{0.7803} & \underline{0.4003} & \underline{0.4473} & \underline{0.3800}
% & 0.7829 & 0.3267 & 0.3966 & 0.4138 \\

% \midrule

% \multirow{8}{*}{\begin{turn}{30}Ours\end{turn}}

% & \darfcnn
% & \multirow{3}{*}{0.7824} & 0.2300 & 0.2496 & 0.1847
% & \multirow{3}{*}{0.7900} & 0.4020 & 0.4485 & 0.3821
% & \multirow{3}{*}{0.7972} & 0.3315 & 0.4026 & 0.4170 \\

% & \darfcnn-\rrf
% & & 0.2339 & 0.2508 & 0.1850
% & & 0.4082 & 0.4511 & 0.3852
% & & 0.3352 & 0.4073 & 0.4177 \\

% & \darfcnn-CC
% & & 0.2412 & 0.2538 & 0.1862
% & & 0.4101 & 0.4519 & 0.3873
% & & 0.3361 & 0.4081 & 0.4200 \\

% \cmidrule(r){2-2}

% & \darfbert
% & \multirow{3}{*}{\textbf{0.8006}$^*$} & 0.2437 & 0.2582 & 0.1886
% & \multirow{3}{*}{\textbf{0.8014}$^*$} & 0.4186 & 0.4544 & 0.3901
% & \multirow{3}{*}{\textbf{0.8081}$^*$} & 0.3330 & 0.4054 & 0.4181 \\

% & \darfbert-\rrf
% & & 0.2462 & 0.2591 & 0.1891
% & & 0.4225 & 0.4558 & 0.3935
% & & 0.3401 & 0.4071 & 0.4203 \\

% & \darfbert-CC
% & & \textbf{0.2526}$^*$ & \textbf{0.2619}$^*$ & \textbf{0.1915}$^*$
% & & \textbf{0.4307}$^*$ & \textbf{0.4586}$^*$ & \textbf{0.3951}$^*$
% & & \textbf{0.3427}$^*$ & \textbf{0.4117}$^*$ & \textbf{0.4236}$^*$ \\

% \midrule

% \multirow{2}{*}{\begin{turn}{30}Ablations\end{turn}}

% & \darfbert-CC-NoQE
% & 0.7722 & 0.2286 & 0.2482 & 0.1845
% & 0.7789 & 0.3911 & 0.4463 & 0.3784
% & 0.7883 & 0.3289 & 0.3980 & 0.4136 \\

% & \darfcnn-CC-NoQE
% & 0.7689 & 0.2207 & 0.2476 & 0.1843
% & 0.7670 & 0.3943 & 0.4433 & 0.3778
% & 0.7858 & 0.3284 & 0.3971 & 0.4140 \\

% \midrule

% & Oracle
% & \cellcolor{ashgrey}1.0000 & \cellcolor{ashgrey}0.2567 & \cellcolor{ashgrey}0.2680 & \cellcolor{ashgrey}0.1942
% & \cellcolor{ashgrey}1.0000 & \cellcolor{ashgrey}0.4394 & \cellcolor{ashgrey}0.4621 & \cellcolor{ashgrey}0.3989
% & \cellcolor{ashgrey}1.0000 & \cellcolor{ashgrey}0.3500 & \cellcolor{ashgrey}0.4148 & \cellcolor{ashgrey}0.4261 \\

% \bottomrule
% \end{tabular}
% \end{adjustbox}
\end{table*}

==> tables/trecdl_monot5.tex <==
\begin{table*}[t]
\centering
\caption{
\small
A comparative evaluation of different SRF approaches on the TREC DL (2019 and 2020) and MS MARCO Dev-small topic sets.
In addition to BM25, we report results with dense neural IR models, MonoT5 and ColBERT.
The PRF method used for improving the ColBERT results is ColBERT-PRF, whereas for BM25 and MonoT5 results are reported with RLM as the PRF method.
Paired $t$-test ($p$<$0.05$) shows a significant improvement of \darf~over the best performing baselines (comparing bold-faced results with the underlined ones).
}
\label{tab:trecdl}

\begin{adjustbox}{width=0.95\textwidth}
\small
\begin{tabular}{@{}llcccc|cccc@{}}

\toprule
\multicolumn{10}{c}{\textbf{Topic Set: TREC DL 19 and 20}} \\
\midrule
& 
& \multicolumn{4}{c}{MonoT5 ($\phi$: RLM)}
& \multicolumn{4}{c}{MonoT5 ($\phi$: GRF)} \\

\cmidrule(r){3-6}
\cmidrule(r){7-10}

& Methods 
& Accuracy & MAP & nDCG@10 & RR@10
& Accuracy & MAP & nDCG@10 & RR@10 \\

\midrule

\multirow{6}{*}{Baselines}
& No PRF 
& N/A & 0.5062 & 0.6451 & 0.8847
& N/A & 0.0000 & 0.0000 & 0.0000 \\


& PRF 
& N/A & 0.5081 & 0.6463 & 0.8826
& N/A & 0.0000 & 0.0000 & 0.0000 \\

& \rrf
& N/A & 0.5112 & 0.6484 & 0.8827
& N/A & 0.0000 & 0.0000 & 0.0000 \\

& \qppbert
& \underline{0.7963} & \underline{0.5189} & \underline{0.6559} & \underline{0.8854}
& 0.0000 & 0.0000 & 0.0000 & 0.0000 \\

& \mcf
& 0.7789 & 0.5071 & 0.6453 & 0.8812
& 0.0000 & 0.0000 & 0.0000 & 0.0000 \\

& \afr 
& 0.7958 & 0.5180 & 0.6543 & 0.8847
& 0.0000 & 0.0000 & 0.0000 & 0.0000 \\

\midrule

\multirow{2}{*}{Ours}

& \darfbert
& \multirow{2}{*}{\textbf{0.8152}$^*$} & 0.5306 & 0.6640 & 0.8903
& \multirow{2}{*}{0.0000} & 0.0000 & 0.0000 & 0.0000 \\

& \darfbert-\rrf
& & 0.5317 & 0.6659 & 0.8910
& & 0.0000 & 0.0000 & 0.0000 \\

\midrule

& Oracle
& \cellcolor{ashgrey}1.0000 
& \cellcolor{ashgrey}0.5416 
& \cellcolor{ashgrey}0.6686
& \cellcolor{ashgrey}0.8937
& \cellcolor{ashgrey}1.0000 
& \cellcolor{ashgrey}0.0000 
& \cellcolor{ashgrey}0.0000
& \cellcolor{ashgrey}0.0000\\

\bottomrule                     
\end{tabular}
\end{adjustbox}
\end{table*}
